Interacting Large Language Model Agents. Interpretable Models and Social Learning

This paper discusses the theory and algorithms for interacting large language model agents (LLMAs) using methods from statistical signal processing and microeconomics. While both fields are mature, their application to decision-making involving interacting LLMAs remains unexplored. Motivated by Bayesian sentiment analysis on online platforms, we construct interpretable models and algorithms that enable LLMAs to interact and perform Bayesian inference. Because interacting LLMAs learn from both prior decisions and external inputs, they can exhibit bias and herding behavior. Thus, developing interpretable models and stochastic control algorithms is essential to understand and mitigate these behaviors. This paper has three main results. First, we show using Bayesian revealed preferences from microeconomics that an individual LLMA satisfies the necessary and sufficient conditions for rationally inattentive (bounded rationality) Bayesian utility maximization and, given an observation, the LLMA chooses an action that maximizes a regularized utility. Second, we utilize Bayesian social learning to construct interpretable models for LLMAs that interact sequentially with each other and the environment while performing Bayesian inference. Our proposed models capture the herding behavior exhibited by interacting LLMAs. Third, we propose a stochastic control framework to delay herding and improve state estimation accuracy under 2 settings: (a) centrally controlled LLMAs (b) autonomous LLMAs with incentives. We demonstrate the effectiveness of our methods on real datasets for hate speech classification and product quality assessment, using open-source models like LLaMA and closed-source models like ChatGPT. The main takeaway of this paper, based on empirical analysis and mathematical formalism, is that LLMAs act as rationally bounded Bayesian agents that exhibit social learning when interacting.

==> draft.tex <==
A recent example of a social sensor is a large language model (LLM) such as GPT, which
utilizes a transformer neural network architecture with billions of parameters. It is predicted
that more than 90\% of web content will eventually be generated by LLMs, as they interact with
one another. Constructing interpretable social learning models for interacting LLMs
is essential for analyzing and controlling their behavior.

We consider the application of LLMs being used to identify if there is  a hate speech peddler in a large group of users that generates content regularly. The content comprises a large corpus of data comprising tweets, blogs, pictures, essays, opinions, etc. However, each LLM charges per token of usage and also has latency constraints. Therefore, it is necessary to use multiple LLM agents that interact with each other as they parse the large corpus of information. Moreover, since LLMs can be fine-tuned for different tasks, a diverse set of LLMs can lead  to an improved performance. To achieve this task, each agents needs to have a Bayesian engine (probabilistic neural network) to compute the posterior distribution of whether the user is a hate speech peddler. Therefore we have a multi-agent social learning framework. 

The unobserved finite state $\state\in \{1,2\}$ is the ground truth of whether the user is a hate speech peddler or not. The observations $z_k$ are the text content generated by the user. When the each LLM agent receives $z_k$, the LLM parses $z_k$ to generate a low dimensional observation $y_k$. This low dimensional representation is designed by the analyst in order to detect hate speech. This observation is fed into the Bayesian engine which generates a posterior of the state. Based on the posterior, the LLM agents optimizes an expected cost which can either be a type-1 error cost ($E(1(x=hate|y_k))$) or could be a more sophisticated sociological cost (details omitted). Using the optimized expected cost, Then the agent selects an action to either flag the user as a hate speech peddler or not.  This action is then broadcast to subsequent LLM agents who parse other portions of the content. The LLM agents share their actions and not the private observations $y_k$ since $y_k$ can reveal private information to the third party services providing the LLM agents. 

Each agent has 3 inputs comprising the action of the previous agent, tokens (i.e. content), a system prompt specifying the task and guidleines for generating the low dimensional representation for the LLM. Each agent has one output, namely, its action. Each LLM has 3 inputs: token, system prompt, side information (e.g., in context training examples). Each LLM agent outputs the low dimensional output $y_k$ as a JSON formatted file.

--------  ----  ----------------------------------------  
